Plato: Approximate Analytics over Compressed Time Series with Tight Deterministic Error Guarantees

Plato provides fast approximate analytics on time series, by precomputing and storing compressed time series. Plato's key novelty is the delivery of tight deterministic error guarantees for time series analytics. Plato evaluates any time series expression composed by the linear algebra operators over vectors, along with arithmetic operators. This large scope of possible expressions includes common use cases such as correlation and cross-correlation expressions. Each time series is segmented either by fixed-length segmentation or by (a usually more effective) variable-length segmentation. Each segment is compressed by an estimation/compression function that approximates the actual values and is coming from a user-chosen function family, as taught by many prior works. The novelty is that Plato associates to each segment 1 to 3 (depending on the case) precomputed error measures and, using them, Plato computes tight deterministic error guarantees for analytics over the compressions. Importantly, some compression families lead to much better deterministic error guarantees. This work identifies two broad estimation function family groups (Vector Space (VS) and Linear Scalable Family (LSF)), which lead to theoretically and practically high-quality guarantees, even for expressions (eg correlation) that combine multiple time series that have been independently compressed and may, thus, use misaligned segmentations. The theoretical aspect of "high quality" is crisply captured by the Amplitude Independence (AI) property: An AI guarantee does not depend on the amplitude of the involved time series, even when we combine multiple time series. The experiments on four real-life datasets showed that when the novel AI guarantees were applicable, the approximate query results were certified to be very close (typically 1%) to the true results.

==> src/copyright.tex <==

% Copyright
%\setcopyright{none}
\setcopyright{acmcopyright}
%\setcopyright{acmlicensed}
%\setcopyright{rightsretained}
%\setcopyright{usgov}
%\setcopyright{usgovmixed}
%\setcopyright{cagov}
%\setcopyright{cagovmixed}

% DOI
\acmDOI{10.475/123_4}

% ISBN
\acmISBN{123-4567-24-567/08/06}

%Conference
\acmConference[SIGMOD'19]{June 2019}{Amsterdam, The Netherlands}

\acmYear{2019}
\copyrightyear{2019}


%\acmArticle{4}
\acmPrice{15.00}

% These commands are optional
%\acmBooktitle{Transactions of the ACM Woodstock conference}
%\editor{Jennifer B. Sartor}
%\editor{Theo D'Hondt}
%\editor{Wolfgang De Meuter}

==> src/keywords.tex <==
%
% The code below should be generated by the tool at
% http://dl.acm.org/ccs.cfm
% Please copy and paste the code instead of the example below.
%

% \begin{CCSXML}
% <ccs2012>
% <concept>
% <concept_id>10002951.10002952</concept_id>
% <concept_desc>Information systems~Data management systems</concept_desc>
% <concept_significance>500</concept_significance>
% </concept>
% <concept>
% <concept_id>10002951.10003317</concept_id>
% <concept_desc>Information systems~Information retrieval</concept_desc>
% <concept_significance>300</concept_significance>
% </concept>
% </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Information systems~Data management systems}
% \ccsdesc[300]{Information systems~Information retrieval}


\keywords{Approximate query processing, Error guarantees}
